Spin conductance in SNN junctions with non-centrosymmetric superconductors

An SNN-junction in which the superconducting potential is a mixture between s-wave and p-wave potentials is investigated using the Usadel equation equipped with Tanaka-Nazarov boundary conditions. The article provides several ways to distinguish between s + chiral and s + helical p-wave superconductors and a way to determine whether a superconductor has a mixed pair potential. Thus, it is of great importance in the determination of the pair potential of superconductors. It is shown that the different spin sectors satisfy independent equations and can thus be calculated separately even if the d-vector depends on the direction of momentum. This greatly simplifies the equations to be solved. It was found that a difference in conductance for sectors with opposite spins arises if both an s-wave and a p-wave component is present, even in the absence of a magnetic field. The results are confirmed by calculations in the ballistic regime. It is shown that the spin conductance for s + chiral p-wave and s + helical p-wave junctions is qualitatively similar. A setup containing two SN junctions is shown to give a clear difference between the two types of superconductivity.

==> Chiequation.tex <==
\section{The phase equation in two dimensions}\label{sec:chiNUM2D}
The expression for the potentially complex phase $\chi$ in the junction is a more difficult problem for quasi-one-dimensional junctions than for one-dimensional junctions. For one-dimensional junctions an analytic expression was found by requiring the $\tau_{3}$-component of $I$ to be 0. In quasi-one-dimensional junctions this is also possible, however, the current is now an average over the nodes. The resulting expression is equation \ref{eq:chiequation2D}:
\begin{align}
 &\int_{-\frac{\pi}{2}}^{\frac{\pi}{2}}\Big((1+T_{1}^{2})(1+g_{+}g_{-}  -f_{+}f_{-})+T_{1} ((g_{+}+g_{-})\cosh{\theta}\nonumber\\&- (f_{+}+f_{-}-(g_{-}f_{+}-g_{+}f_{-}) )e^{i(\psi-\chi)}\sinh{\theta}- (f_{+}+f_{-}+(g_{-}f_{+}-g_{+}f_{-}) )e^{-i(\psi-\chi)}\sinh{\theta} )\Big)^{-1}\nonumber\\&e^{i(\psi-\chi)}(f_{+}+f_{-}-(g_{-}f_{+}-g_{+}f_{-})) - e^{i(\chi-\psi)}(f_{+}+f_{-}+(g_{-}f_{+}+g_{+}f_{-}))T\cos{\phi} d\phi \nonumber \\&=0,\label{eq:chiequation2D}
\end{align}
where
\begin{align}
    g_{\pm}(\phi) &= \frac{E}{\sqrt{E^{2}-\Delta_{\pm}(\phi)}}\\
    f_{\pm}(\phi) &= \frac{\Delta_{\pm}(\phi)}{\sqrt{E^{2}-\Delta_{\pm}(\phi)}}\\
    \Delta_{\pm}(\phi)& \frac{1}{\sqrt{r^{2}+1}}\pm\frac{r}{\sqrt{r^{2}+1}}\cos{\phi},\\
    T(\phi) &= \frac{\cos^{2}\phi}{\cos^{2}{\phi}+(\frac{z}{2})^{2}},\\
    T_{1}(\phi) &= \frac{T(\phi)}{2-T(\phi)+2\sqrt{1-T(\phi)}}.
\end{align}
A big difference with the expression for the one-dimensional junction is that the phase in the junction depends on the parameter $\theta$. Instead of finding the analytical solution to equation \ref{eq:chiequation2D}, a numerical procedure was developed. Denote the integral in equation \ref{eq:chiequation2D} by $S_{\phi}$. The condition can then be shortly written as 
\begin{equation}
    S_{\phi}(\theta,\chi) = 0.
\end{equation}
Now start from an initial guess $\chi_{i}$ and denote the new guess $\chi_{i+1} = \chi_{i}+\delta\chi$. Then $\delta\chi$ is chosen such that
\begin{equation}
    S_{\phi}(\theta,\chi_{i+1})\approx S_{\phi}(\theta,\chi_{i})+\dv{S_{\phi}}{\chi}\delta\chi = 0,
\end{equation}
that is
\begin{equation}
    \delta\chi = -\frac{1}{S_{\phi}}\dv{S_{\phi}}{\chi}.
\end{equation}
The quantity $\dv{S}{\chi}$ can be calculated to be
\begin{align}
    \dv{S}{\theta} =& 2T\left((2-T)\mathbf{1}+T(CG+GC)\right)^{-1}\left(C\dv{G}{\chi}-\dv{G}{\chi}C\right)\nonumber\\+&2T\left((2-T)\mathbf{1}+T(CG+GC)\right)^{-1}\left((2-T)\mathbf{1}+T(C\dv{G}{\chi}+\dv{G}{\chi}C)\right)\nonumber\\&\left((2-T)\mathbf{1}+T(CG+GC)\right)^{-1}\left(CG-GC\right),\\
    \dv{G}{\chi} =& \begin{bmatrix}0&i\sinh{\theta}e^{i\chi}\\i\sinh{\theta}e^{-i\chi}&0\end{bmatrix}.
\end{align}
This procedure was repeated was repeated until $S_{\phi}$ was lower than the tolerance. It was found that this procedure converges well if one takes for the first initial guess $\chi_{0}$ the phase in the one-dimensional junction using the same parameters. Once there was solved for the parameter $\chi$, the parameter $\theta$ was recalculated by solving the Usadel equation using the same method as for one-dimensional junction.\\
This procedure was found to work well for $r<0.95$ and $r>1.5$. When $r$ is close to 1, the code has trouble with convergence. These convergence issues can be traced back to the one-dimensional case, where $r = 1$ can not be solved using the $\theta$-parametrisation, and where near $r = 1$ the imaginary part of $\chi$ can become large. For spin up electrons this imaginary part is positive, for spin down electrons this imaginary part is negative. Therefore, for the solution of $S_{\phi}(\theta,\chi) = 0$ the parameter $X_{\uparrow,\downarrow}$ was introduced:
\begin{align}
    X_{\uparrow} &= \sinh{\theta_{\uparrow}}e^{-i\chi}\\
    X_{\downarrow}  &=\sinh{\theta_{\downarrow}}e^{i\chi}\\
    G_{\uparrow}& = \begin{bmatrix}\cosh{\theta_{\uparrow}}&\frac{\sinh^{2}{\theta_{\uparrow}}}{X_{\uparrow}}\\-X_{\uparrow}&-\cosh{\theta_{\uparrow}}\end{bmatrix}\\
    G_{\downarrow}& = \begin{bmatrix}\cosh{\theta_{\downarrow}}&X_{\downarrow}\\-\frac{\sinh^{2}{\theta_{\downarrow}}}{X_{\downarrow}}&-\cosh{\theta_{\downarrow}}\end{bmatrix}.
\end{align}
Contrary to the parameter $\chi$ the parameter $X$ does not become very large. Using this procedure also $0.95<r<1$ and $1<r<1.5$ could be calculated.

==> Chiral.tex <==
\section{Twodimensional s + chiral p-wave junction}
Now that s + $\text{p}_{\text{x}}$ wave superconductor junctions have been studied, also other, similar junctions can be studied, such as the s + chiral p-wave superconductor. 
In a chiral p-wave superconductors there are no nodes \cite{kallin2016chiral}, that is, angles $\phi$ such $\Delta(\phi) = 0$, contrary to the p-wave superconductor studied before. They are topologically nontrivial \cite{schnyder2008classification}, that is, there is a quantised quantity, called the winding number \cite{schnyder2008classification}, that takes a different value in a chiral superconductor than it does in normal metals. For detailed discussions of the winding number and the connection with the emergence of Majorana fermions, the reader is referred to \cite{kallin2016chiral}, \cite{schnyder2008classification}, and sources therein. For pure p-wave superconductors, the Andreev bound states have flat dispersion if the superconductor is not chiral, and non-flat dispersion if the superconductor is chiral.\\
In the clean limit, junctions with s + chiral p-wave junction have been theoretically investigated in \cite{burset2014transport}, where it was shown that Andreev bound states with non-flat dispersion exist if the chiral p-wave component of the pair potential is dominant, whereas they are absent if the s-wave component is dominant.
\\
 In this section differences in the density of states, pair amplitude and conductance between dirty SNN junctions with mixed s + chiral p-wave superconductors and mixed s + non-chiral p-wave superconductors will be investigated.\\
In a chiral p-wave superconductor the superconductor pair potential and corresponding retarded Green's function are given by \cite{sawa2007quasiclassical}:
\begin{align}
    \Delta_{cp}(\phi) &= e^{i\phi},
    G_{S}=\begin{bmatrix}\frac{E}{\sqrt{E-|\Delta_{cp}(\phi)|^2}}&\frac{\Delta_{cp}}{\sqrt{E-|\Delta_{cp}(\phi)|^2}}\\-\frac{\Delta_{cp}^{*}}{\sqrt{E-|\Delta_{cp}(\phi)|^2}}&-\frac{E}{\sqrt{E-|\Delta_{cp}(\phi)|^2}}\end{bmatrix}.
\end{align}
Therefore, in the s + chiral p-wave superconductor, the following potential will be used:
\begin{align}
    \Delta = \frac{1}{\sqrt{r^{2}+1}}+\frac{r}{\sqrt{r^{2}+1}}e^{i\phi},
    G_{S}=\begin{bmatrix}\frac{E}{\sqrt{E-|\Delta(\phi)|^2}}&\frac{\Delta}{\sqrt{E-|\Delta(\phi)|^2}}\\-\frac{\Delta^{*}}{\sqrt{E-|\Delta(\phi)|^2}}&-\frac{E}{\sqrt{E-|\Delta(\phi)|^2}}\end{bmatrix}.
\end{align}
Note that $\Delta(0) = \frac{1}{\sqrt{r^{2}+1}}+\frac{r}{\sqrt{r^{2}+1}}$ and $\Delta(\pi) = \frac{1}{\sqrt{r^{2}+1}}-\frac{r}{\sqrt{r^{2}+1}}$, just as for the s + p-wave superconductor. In the purely one dimensional junction, the s + chiral p-wave superconductor gives the same results as the s + p wave superconductor. In the coming section the behaviour in the quasi-one-dimensional superconductor is investigated.\\
The procedure to find the solutions to the equation is the same as for s + p-wave superconductors. The results are shown in figure \ref{fig:Fcr}. The results are similar to the s + p-wave junction. Also here, there are only two non-vanishing components, of which the singlet is dominant if $r<1$ and the triplet is dominant if $r>1$. A difference with the s + p-wave junction is that the non-dominant component is much larger for the s + chiral p-wave junction. Moreover, the zero energy non-dominant component is now nonvanishing on $(0,\infty)$ instead of $(1,\infty)$. This difference arises because $\Delta_{\pm}$ are not on the positive real axis anymore in general. This difference also appears in the density of states, as shown in figures \ref{fig:rhochiral} and \ref{fig:rhochiralSP}. Just as in the junctions studied in previous sections, there is a zero energy dip in the density of states for $r < 1$ and a zero energy peak for $r > 1$. However, contrary to the quasi one dimensional s + p-wave junction, the magnitude of the dip for $r<1$ now depends on the actual value that $r$ takes. This can be explained from the discussion in supplementary material \ref{sec: Very low energy}. There, it is shown that the low energy behaviour is determined by $\frac{\Delta_{+}(\phi)}{|\Delta_{+}(\phi)|}$ and $\frac{\Delta_{+}(\phi)}{|\Delta_{+}(\phi)|}$. For the s + $\text{p}_{\text{x}}$-wave junction the quantities $\frac{\Delta_{\pm}}{|\Delta_{\pm}|}$ were on the positive real axis independent of $\phi$ if $r<1$, and thus, both quantities were 1 for all angles, independent of $r$. For the s + chiral p-wave junction this is not the case any more, so $\frac{\Delta_{\pm}(\phi)}{|\Delta_{\pm}(\phi)|}$ will be different from 1, and depend on the actual value of $r$.
\begin{figure}
    \centering
\subcaptionbox{$r = 0.2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fcr0p2.png}}
\hfill
\subcaptionbox{$r = 2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fcr2.png}}

    \caption{The singlet and triplet components in the normal metal for different values of $r$ for the quasi-one-dimensional junctions using a chiral p-wave superconductor. The gauge was chosen such that $F_{1}$ corresponds to bulk s-wave superconductors. The results are similar to the results when a normal p-wave superconductor is used, with the exception that for $r>1$, the singlet component now attains a maximum at zero energy.}
    \label{fig:Fcr}
\end{figure}
\begin{comment}
\begin{figure}
    \centering
    \subcaptionbox{$r = 0$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fcr0.png}}
\hfill
\subcaptionbox{$r = 0.2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fcr0p2.png}}
\hfill
\subcaptionbox{$r = 0.9$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fcr0p9.png}}
\hfill
\subcaptionbox{$r = 2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fcr2.png}}
\hfill
\subcaptionbox{$r = 5$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fcr5.png}}
\hfill
\subcaptionbox{$r = \infty$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/FcrInf.png}}
    \caption{The singlet and triplet components in the normal metal for different values of $r$ for the quasi-one-dimensional junctions using a chiral p-wave superconductor. The gauge was chosen such that $F_{1}$ corresponds to bulk s-wave superconductors. The results are similar to the results when a normal p-wave superconductor is used, with the exception that for $r>1$, the singlet component now attains a maximum at zero energy.}
    \label{fig:Fcr}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width = 0.7\textwidth]{figures/nondominantchiral.png}
    \caption{The non-dominant component at zero energy for different values of $r$. There are two major differences with the s + p-wave case. First, the non-dominant component at zero energy is much larger for s + chiral p-wave superconductors. Second, whereas for the s + p-wave superconductors the non-dominant component at zero energy vanished exactly, for s + chiral p-wave superconductors the non-dominant component is non-vanishing for $r\in(0,\infty)$. The divergence at $r = 1$ is clearly visible.}
    \label{fig:Nondominantchiral}
\end{figure}
\end{comment}
\begin{figure}
    \centering
    \includegraphics[width = 0.7\textwidth]{figures/rhochiral.png}
    \caption{The density of states in an s + chiral p-wave junction. When $r<1$ there is a dip in the density of states at zero energy, when $r>1$ there is a peak in the density of states. The density of states is very similar to the density of states in an s + p-wave junction.}
    \label{fig:rhochiral}
\end{figure}
\begin{comment}
\begin{figure}
    \centering
    \subcaptionbox{$r < 1$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/rhochiralS.png}}
\hfill
\subcaptionbox{$r > 1$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/rhochiralP.png}}
    \caption{The density of states in the s + chiral p-wave junction when the s-wave component is dominant (left) and when the p-wave componenent is dominant (right). Contrary to the s + p-wave junction, the magnitude of the zero energy dip depends now on the ratio $r$.}
    \label{fig:rhochiralSP}
\end{figure}
\end{comment}

Next, the conductance in the s + chiral p-wave junction was studied. In its calculation, it should be noted that for chiral p-wave superconductors, using the notation of \cite{tanaka2021phys},
\begin{align}
    f_{+\downarrow}(\phi) &= -\frac{\Delta_{s}-\Delta e^{i\phi}}{\sqrt{E^{2}-|\Delta_{-}|^{2}}} = -f_{-\uparrow}^{*}(\phi) = -f_{-\uparrow}(-\phi),\\
    f_{-\downarrow}(\phi) &= -\frac{\Delta_{s}+\Delta e^{i\phi}}{\sqrt{E^{2}-|\Delta_{+}|^{2}}} = -f_{+\uparrow}^{*}(\phi) = -f_{+\uparrow}(-\phi),
\end{align}
This should be contrasted to the previously studied cases, where, as in \cite{tanaka2021phys}, it holds that
\begin{align}
    f_{+\downarrow}(\phi) &= -f_{-\uparrow}(\phi),\\
    f_{-\downarrow}(\phi) &= -f_{+\uparrow}(\phi).\\
\end{align}
However, for the boundary condition, an angular average is used. Therefore, the procedure as in \cite{tanaka2021phys} can still be followed.
%Therefore, $c_{1\down} = c_{1\up}, c_{2\down} = -c_{2\up}, c_{3\down} = c_{3\up}$ does not hold anymore. However, it does hold that $c_{1\down}(\phi) = c_{1\up}(-\phi), c_{2\down} = -c_{2\up}(-\phi), c_{3\down}(\phi) = c_{3\up}(-\phi)$, and since the contributions from angles $\phi$ and $-\phi$ are summed, the preceding formulas can still be used.
The results are shown in figure \ref{fig:Sigmachiral} and \ref{fig:SigmaeVchiral}. For $r<1$, where the s-wave component is dominant, the results for the s + chiral p-wave junction and for the s + $\text{p}_{\text{x}}$-wave junction are very similar. A difference between the two cases is whereas the zero bias conductance is constant with $r$ for $r<1$ in the s + $\text{p}_{\text{x}}$-wave junction, in the s + chiral p-wave junction a minimum in the zero bias conductance is attained for $\frac{\Delta_{p}}{\Delta_{s}}\approx\frac{2}{3}$, as shown in figure \ref{fig:SigmaeVchiral}. For $r>1$ however, where the chiral p-wave component is dominant, there are significant differences with the s + p-wave junction. Figure \ref{fig:Sigmachiral} shows that for the chiral junction the zero bias conductance peak is significantly suppressed. Moreover, the peak can now be seen as composed from two different peak structures, one narrow peak with width of the order $E_{Th}$, as for the normal p-wave, and one broader peak, which extends to almost $E = \Delta$ for large $r$. This is consistent with the result in \cite{tanaka2005theory} for pure chiral p-wave superconductors, which also shows this double peak structure. Due to the nontrivial dependence of the zero bias conductance for $r<1$, the zero bias conductance does not show a clear discontinuity in the zero bias conductance for the s + chiral p-wave junction, as shown in figure \ref{fig:SigmaeVchiral}.

\begin{figure}
    \centering
    \includegraphics[width = 0.7\textwidth]{figures/ChiralConductance.png}
    \caption{The conductance of the s + chiral p-wave junction.}
    \label{fig:Sigmachiral}
\end{figure}
\begin{figure}
    \centering
    \subcaptionbox{$r = 0$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/SigmachiraleVr.png}}
\hfill
\subcaptionbox{$r = 0.2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/SigmaeV0chiral.png}}

    \caption{The conduction in the quasi-1D SNN junction with a mixed s + chiral P-wave superconductor pair potential as a function of voltage and $\frac{r}{1+r}$. The distinction between the two cases is clearly visible. For $r<1$ there is a dip in the density of states at low energies, for $r>1$ there is a peak at low energies. The width of the peak or dip decreases as the contributions from the s-wave and p-wave component become more equal in strength. The peak at $eV = \Delta$ for s-wave dominant junctions is more clearly visible for the chiral p-wave case than for the $\text{p}_{\text{x}}$-wave case. This is not caused by an enhancement of this peak, but rather by a decrease of the height of the zero bias conductance peak. The conductance at zero energy does not show a discontinuity at $r = 1$. The dependence on $\frac{r}{1+r}$ is similar compared to the s + $\text{p}_{\text{x}}$-wave junction, however, the kink that appeared for the s + $\text{p}_{\text{x}}$-wave is smoothened for the s + chiral p-wave case, in line with the other results. In fact, $\pdv{}{r}\sigma(eV = 0)|_{r = 0}<0$, that is, by adding a chiral p-wave component to the potential the zero bias conductance first decreases and attains a minimum. The minimum was found to be at $\frac{r}{1+r}\approx 0.4$, that is, $r \approx \frac{2}{3}$.}
    \label{fig:SigmaeVchiral}
\end{figure}
\begin{comment}
\subsection{Angular mismatch}
If there is an angular mismatch of $\alpha$, that is, the potential is given by $\Delta = \Delta_{s}+\Delta_{p}e^{i(\phi-\alpha)}$, then
\begin{align}
    f_{+\uparrow}(\phi) &= \frac{\Delta_{s}+\Delta e^{i(\phi-\alpha)}}{\sqrt{E^{2}-|\Delta_{+}|^{2}}}\\
    f_{+\uparrow}(\phi)& = \frac{\Delta_{s}-\Delta_{p}e^{i(-\phi-\alpha)}}{\sqrt{E^{2}-|\Delta_{-}|^{2}}}\\
    f_{+\downarrow}(\phi) &=\frac{-\Delta_{s}+\Delta_{p}e^{i(\phi-\alpha)}}{\sqrt{E^{2}-|\Delta_{-}|^{2}}} = -f_{-\uparrow}(-\phi)\neq f^{*}_{-\uparrow}(\phi)\\
    f_{-\downarrow}(\phi) &=\frac{-\Delta_{s}-\Delta_{p}e^{i(-\phi-\alpha)}}{\sqrt{E^{2}-|\Delta_{-}|^{2}}} = -f_{+\uparrow}(-\phi)\neq f^{*}_{+\uparrow}(\phi)\\
\end{align}
Since the equalities $f_{+\downarrow}(\phi) = -f_{-\uparrow}(-\phi)$ and $f_{-\downarrow}(-\phi) = -f_{+\uparrow}(-\phi)$ are satisfied, the procedure in \cite{tanaka2021phys} can still be followed.
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> Introduction.tex <==
\section{\label{sec:Introduction}Introduction}
The discovery of superconductivity \cite{onnes1911further}, more than a century ago, led to both theoretical and experimental investigations of this phenomenon. 
In the first half century, focus was on what are now called conventional superconductors \cite{LONDON1935341},\cite{ginzburg2004superconductivity}, \cite{BCS1957a}, \cite{BCS1957b}, that is, superconductors in which the superconducting interaction is isotropic \cite{schmidt1997physics}. However, the discovery of high temperature superconductivity \cite{buchholtz1981identification}, \cite{steglich1979superconductivity}, \cite{bednorz1986possible}, brought about the investigation of other types of superconductivity, called unconventional superconductors \cite{sigrist2005review}, \cite{maeno2011evaluation}. These unconventional superconductors are classified in a way similar to the angular momentum states in the 3D harmonic oscillator \cite{griffiths2010introduction}, that is, by p-wave, d-wave, f-wave and further, whereas conventional superconductors are also called s-wave superconductors. The superconductor pair potentials that will be used here are mixtures the isotropic singlet s-wave potential $\Delta_{s} = i\sigma_{y}\Delta_{0}$ and the non-isotropic triplet p-wave potential $\Delta = \Delta_{0} i(d_{x}\sigma_{x}+d_{y}\sigma_{y}+d_{z}\sigma_{z})\sigma_{y}$. The $d$-vector can either be for a $\text{p}_{\text{x}}$-wave $(0,0,\cos{\phi})$, chiral p-wave $(0,0,e^{i\phi})$ or helical p-wave $(\cos{\phi},\sin{\phi},0)$, where $\phi$ is the angle with a specified axis and $\sigma_{x,y,z}$ denote the spin Pauli matrices.
Here $\Delta_{0}$ is an energy scale denoting the strength of the interactions, and $\phi$ is the angle made with an assigned axis. 
\begin{comment}
An illustration of s-wave and $\text{p}_{\text{x}}$-wave superconductivity is shown in figure \ref{fig:potentialSP}.
\begin{figure}
\centering
\begin{tikzpicture}
\filldraw[color=blue!60, fill=blue!5](-1,0) circle (1.5);
\coordinate (G) at (2,0);
\coordinate (R) at (10,0);
\coordinate (B) at (6,0);
\draw[name path = F,blue]   (R) to[out=-90,in=-45] (B);
\draw[name path = H,blue]    (R) to[out=90,in=45] (B);
\draw[name path = I,red]    (G) to[out=-90,in=-135] (B);
\draw[name path = J,red]    (G) to[out=90,in=135] (B);
\tikzfillbetween[of = F and H]{blue,opacity = 0.1};
\tikzfillbetween[of = I and J]{red,opacity = 0.1};
\end{tikzpicture}
\caption{A two dimensional illustration of the pair potentials of s-wave (left) and $\text{p}_{\text{x}}$-wave (right) superconductors. For s-wave superconductors, the pair potential is isotropic, for p-wave superconductors, the pair potential has a strong angle dependence, $\Delta = \Delta_{0}\cos{\phi}$, where $\phi$ is the angle made with a horizontal line. Colour coding has been used to indicate the sign of $\Delta$. Note that a negative sign of $\Delta$ does not mean there is repulsion instead of attraction. \label{fig:potentialSP}}
\end{figure}
\end{comment}
Whereas d-wave superconductivity has been firmly established \cite{hilgenkamp2003ordering}, the experimental verification of existence of p-wave superconductivity is still under debate, a major candidate for p-wave superconductivity being $\text{SrRuO}_{4}$ \cite{maeno2011evaluation}, \cite{suh2020stabilizing}, \cite{kallin2009sr2ruo4}.\\ To investigate the type of superconductivity it is important to realise the superconductor pair potential might not be a pure s-wave, p-wave or d-wave superconductor pair potential, in principle also mixtures are possible. To study the properties of unconventional superconductors and the robustness of these properties when the superconductor pair potential is changed, it is important to understand the properties of superconductors in which the superconductor pair potential is a mixture of the types listed above, such as a mixture between s-wave and p-wave superconductors. In this example, following the notation in \cite{mishra2021effects}, the superconductor pair potential can be written as 
\begin{equation}
    \Delta = \frac{1}{\sqrt{r^{2}+1}}\Delta_{s}+\frac{r}{\sqrt{r^{2}+1}}\Delta_{p},
\end{equation}
where $r$ denotes the relative strength of the s-wave and p-wave contributions to the potential, $\Delta_{s}$ is the s-wave superconductor pair potential, and $\Delta_{p}$ is one of the p-wave superconductor pair potentials.
\begin{comment}
A schematic of the mixed potential is shown in figure \ref{fig:potentialSPmix} in the case of a s + $\text{p}_{\text{x}}$-wave superconductor.
\begin{figure}
\centering
\begin{tikzpicture}
\draw[dashed](-1,0) circle (1.5);
\draw[dashed](6,0) circle (0.5);
\coordinate (GS) at (-2,0);
\coordinate (RS) at (1,0);
\coordinate (BS) at (-1,0);
\coordinate (US) at (-1,1.5);
\coordinate (DS) at (-1,-1.5);
\draw[name path = FS,blue] (GS) to[out=90,in=190] (US);
\draw[name path = HS,blue] (US) to[out=10,in=90]  (RS);
\draw[name path = IS,blue] (GS) to[out=-90,in=170] (DS);
\draw[name path = JS,blue] (DS) to[out=-10,in=-90]  (RS);
\tikzfillbetween[of = FS and IS]{blue,opacity = 0.1};
\tikzfillbetween[of = HS and JS]{blue,opacity = 0.1};
\coordinate (G) at (5,0);
\coordinate (R) at (8,0);
\coordinate (B) at (6,0);
\coordinate (U) at (6,0.5);
\coordinate (D) at (6,-0.5);
\draw[name path  = K, blue] (U) to[out = -160, in = 135] (B);
\draw[name path = L, blue] (U) to[out = 20, in = 90] (R);
\draw[name path  = F, blue] (D) to[out = 160, in = -135] (B);
\draw[name path = H, blue] (D) to[out = -20, in = -90] (R);
\draw[name path = I,red]    (G) to[out=-90,in=-135] (B);
\draw[name path = J,red]    (G) to[out=90,in=135] (B);
\tikzfillbetween[of = F and K]{blue,opacity = 0.1};
\tikzfillbetween[of = H and L]{blue,opacity = 0.1};
\tikzfillbetween[of = I and J]{red,opacity = 0.1};
\end{tikzpicture}
\caption{A two dimensional illustration of the pair potentials of a s + $\text{p}_{\text{x}}$ - wave superconductor, in which respectively s-wave (left) and p-wave (right) are the dominant pair potential. In both cases the dominant pair potential is three times as large as the non-dominant pair potential. For comparison the s-wave component is shown as a dotted line for both cases.  Colour coding has been used to indicate the sign of $\Delta$. Note that a negative sign of $\Delta$ does not mean there is repulsion instead of attraction. If the s-wave component is dominant the sign of $\Delta$ is the same for all angles, if the p-wave component is dominant there is a sign change. \label{fig:potentialSPmix}}
\end{figure}
\end{comment}
One way to investigate the properties of superconductors is by studying systems in which a superconducting material is in contact with a material that by itself is not a superconductor. Interest in those systems has risen since the prediction \cite{josephson1962possible} and experimental verification \cite{josephson1965supercurrents} of the Josephson effect. Josephson showed \cite{josephson1962possible} that in an SNS junction, that is, a junction made by sandwiching a non superconducting material between two superconductors, there can still be a supercurrent, a dissipationless current. Thus, the proximity of a superconductor influences the electronic properties of other materials. This is called the proximity effect \cite{schmidt1997physics}.\\ 
The proximity effect can be studied in SNS junctions, but also in SNN junctions, in which a normal metal is sandwiched between a superconductor and another normal metal. In this case there is no supercurrent \cite{schmidt1997physics}, but the superconductor will still influence the normal metal. To distinguish the 'middle N' from the 'right N', the 'middle N' will be called the normal metal bar, whereas the 'right N' will be referred to as the normal metal electrode.  In this article, the properties of the normal metal bar will be investigated for proximity structures with different superconductor pair potentials.\\
The method that will be used is the Keldysh Green's function technique, with $G = \begin{bmatrix}G_{R}&G_{K}\\0&G_{A}\end{bmatrix}$, where $G_{R}, G_{A}, G_{K}$ are the retarded, Keldysh and advanced parts respectively, which are all four by four matrices to take into account spin space as well as the particle hole space


==> Keldysh.tex <==
\begin{widetext}
\section{Keldysh equation}\label{sec:Keldyshequation}
In this section the equations for the Keldysh equations will be calculated. It will be shown that in case a complex superconducting phase $\chi$ in the normal layer is allowed, additional terms occur compared to expressions previously noted in literature \cite{brinkman2003microscopic}, \cite{belzig1999quasiclassical}. Recall that the Usadel equation reads
\begin{equation}
    \pdv{}{x}\left(G\pdv{G}{x}\right)+i\epsilon [G,\tau_{3}]+2\Theta_{S}[G,B] = 0.
\end{equation}
Moreover, for any matrix $Z$ consisting of a retarded, advanced and Keldysh components we can write $Z_{K} = Z_{R}h-hZ_{A}$ where $h$ is a diagonal matrix. In the following chapters, $h$ will be used in the normal metal, whereas $h_{s}$ will be used in the superconducting electrodes.
First the Keldysh component of the first term will be calculated.
\begin{equation}
\begin{split}
    (G\nabla G)_{K}&= G_{R}\nabla G_{K} + G_{K}\nabla G_{A}=G_{R}\nabla(G_{R}h-hG_{A})+(G_{R}h-hG_{A})\nabla G_{A}\\& =G_{R}\nabla G_{R}h+G_{R}^{2}\nabla h -G_{R}\nabla h G_{A}-G_{R}h\nabla G_{A}+G_{R}h\nabla G_{A}-hG_{A}\nabla G_{A}\\
    & = \nabla h-G_{R}\nabla h G_{A}+G_{R}\nabla G_{R} h - hG_{A}\nabla G_{A}.\\
\end{split}
\end{equation}
Thus, the Keldysh equation reads
\begin{equation}
    \begin{split}
        &\nabla (\nabla h-G_{R}\nabla h G_{A})+\nabla(G_{R}\nabla G_{R})h+G_{R}\nabla G_{R} \nabla h - h\nabla(G_{A}\nabla G_{A})-\nabla h G_{A}\nabla G_{A}\\&+i\epsilon( [G_{R},\tau_{3}]h-h[G_{A},\tau_{3}])+2[G,B]_{K}\Theta_{S}(x) = 0.
    \end{split}
\end{equation}
Now, adding and subtracting $2([G,B]_{R}h-h[G,B]_{A})\Theta_{s}(x)$ and rearranging the terms this can be written as
\begin{equation}
    \begin{split}
        &\nabla (\nabla h-G_{R}\nabla h G_{A})+\left(\nabla(G_{R}\nabla G_{R})+i\epsilon [G_{R},\tau_{3}]+2[G,B]_{R}\Theta_{s}(x)\right)h+G_{R}\nabla G_{R} \nabla h \\&- h\left(\nabla(G_{A}\nabla G_{A})+i\epsilon [G_{A},\tau_{3}]+2[G,B]_{A}\right)-\nabla h G_{A}\nabla G_{A}+2([G,B]_{K}-[G,B]_{R}h+h[G,B]_{A})\Theta_{s}(x) = 0.
    \end{split}
\end{equation}
Now, using the retarded and advanced components two of these expressions can be seen to vanish, and the equation left is
\begin{equation}\label{eq:KeldyshS}
    \begin{split}
        0 = & \nabla (\nabla h-G_{R}\nabla h G_{A})+G_{R}\nabla G_{R} \nabla h -\nabla h G_{A}\nabla G_{A}+2([G,B]_{K}-[G,B]_{R}h+h[G,B]_{A})\Theta_{s}(x).\\=&\nabla (\nabla h-G_{R}\nabla h G_{A})+G_{R}\nabla G_{R} \nabla h -\nabla h G_{A}\nabla G_{A}+S = 0,\\
        S=&2([G,B]_{K}-[G,B]_{R}h+h[G,B]_{A})\Theta_{s}(x).
    \end{split}
\end{equation}
Now writing $h = f_{L}\tau_{0}+f_{T}\tau_{3}$ this becomes
\begin{eqnarray}
    &\nabla\left((1-G_{R}G_{A})\nabla f_{L}\right)+\nabla\left((\tau_{3}-G_{R}\tau_{3}G_{A})\nabla f_{T}\right)+\nabla f_{L} (G_{R}\nabla G_{R}-G_{A}\nabla G_{A})\nonumber\\&+\nabla f_{T} (G_{R}\nabla G_{R}\tau_{3}-\tau_{3}G_{A}\nabla G_{A})+S =0.\label{eq:Keldyshnopar}
\end{eqnarray}
Now, the terms in equation \ref{eq:Keldyshnopar} need to be calculated.
\subsubsection{Calculation of terms}
The first term in equation \ref{eq:Keldyshnopar} is $1-G_{R}G_{A} = 1+G_{R}\tau_{3}G_{R}^{\dagger}\tau_{3}$.
Using that 
\begin{equation}
    G_{R} = \begin{bmatrix}\cosh{\theta}&\sinh{\theta}e^{i\chi}\\-\sinh{\theta}e^{-i\chi}&-\cosh{\theta}\end{bmatrix},
\end{equation}
it follows that 
\begin{equation}
    \tau_{3}G_{R}^{\dagger}\tau_{3} = \begin{bmatrix}\cosh{\theta^{*}}&\sinh{\theta^{*}}e^{i\chi^{*}}\\-\sinh{\theta^{*}}e^{-i\chi^{*}}&-\cosh{\theta^{*}}\end{bmatrix},
\end{equation}
and therefore that
\begin{equation}
    G_{R}\tau_{3}G_{R}^{\dagger}\tau_{3} = \begin{bmatrix}|\cosh{\theta}|^{2}-|\sinh{\theta}|^{2}e^{-2\text{Im}\chi}&\cosh{\theta}\sinh{\theta^{*}}e^{i\chi^{*}}-\cosh{\theta^{*}}\sinh{\theta}e^{i\chi}\\ \cosh{\theta}\sinh{\theta^{*}}e^{-i\chi^{*}}-\cosh{\theta^{*}}\sinh{\theta}e^{-i\chi}&|\cosh{\theta}|^{2}-|\sinh{\theta}|^{2}e^{2\text{Im}\chi}\end{bmatrix}
\end{equation}
Thus, define
\begin{equation}\label{eq:DLdef}
    D_{L} = Tr(1-G_{R}G_{A}) = 2+2|\cosh{\theta}|^{2}-2|\sinh{\theta}|^{2}\cosh{2\text{Im}\chi},
\end{equation}
and
\begin{equation}\label{eq:CTdef}
    C_{T} = Tr(\tau_{3}-\tau_{3}G_{R}G_{A}) = 2|\sinh{\theta}|^{2}\sinh{2\text{Im}\chi}.
\end{equation}
\\
For the second term note that $-G_{R}\tau_{3}G_{A} = G_{R}G_{R}^{\dagger}\tau_{3}$. This can be calculated and yields
\begin{equation}
\begin{split}
    G_{R}G_{R}^{\dagger}\tau_{3} &= \begin{bmatrix}\cosh{\theta}&\sinh{\theta}e^{i\chi}\\-\sinh{\theta}e^{-i\chi}&-\cosh{\theta}\end{bmatrix}\begin{bmatrix}\cosh{\theta^{*}}&\sinh{\theta^{*}}e^{i\chi^{*}}\\\sinh{\theta^{*}}e^{-i\chi^{*}}&\cosh{\theta^{*}}\end{bmatrix}\\&=\begin{bmatrix}|\cosh{\theta}|^{2}+|\sinh{\theta}|^{2}e^{-2\text{Im}\chi}&\cosh{\theta}\sinh{\theta^{*}}e^{i\chi^{*}}+\cosh{\theta^{*}}\sinh{\theta}e^{i\chi}\\ -\cosh{\theta}\sinh{\theta^{*}}e^{-i\chi^{*}}-\cosh{\theta^{*}}\sinh{\theta}e^{-i\chi}&-|\cosh{\theta}|^{2}-|\sinh{\theta}|^{2}e^{2\text{Im}\chi}\end{bmatrix}
\end{split}
\end{equation}
Thus, define
\begin{equation}\label{eq:CLdef}
    C_{L} = Tr(\tau_{3}-G_{R}\tau_{3}G_{A}) = -2|\sinh{\theta}|^{2}\sinh{2\text{Im}\chi} = -C_{T},
\end{equation}
and
\begin{equation}\label{eq:DTdef}
    D_{T} = Tr(1-\tau_{3}G_{R}\tau_{3}G_{A}) =2+2|\cosh{\theta}|^{2}+2|\sinh{\theta}|^{2}\cosh{2\text{Im}\chi}.
\end{equation}
\\
The third term reads $G_{R}\nabla G_{R}\tau_{3}-\tau_{3}G_{A}\nabla G_{A}$.
Now,
\begin{equation}
    \begin{split}
        G_{R}\nabla G_{R}& = \begin{bmatrix}0 &e^{i\chi}\\e^{-i\chi}&0\end{bmatrix}\pdv{\theta}{x}\nonumber\\&+\begin{bmatrix}i\sinh^{2}{\theta}&i\cosh{\theta}\sinh{\theta}e^{i\chi}\\-i\cosh{\theta}\sinh{\theta}e^{-i\chi}&-i\sinh^{2}{\theta}\end{bmatrix}\pdv{\chi}{x}.
    \end{split}
\end{equation}
From this it can be calculated that
\begin{equation}\label{eq:GRnablaGR}
    \begin{split}
        &\text{Tr}(G_{R}\nabla G_{R}) = 0,\\
        &\text{Tr}(\tau_{3}G_{R}\nabla G_{R}) = 2i\sinh^{2}{\theta}\pdv{\chi}{x}.
    \end{split}
\end{equation}
Similarly, for $G_{A}\nabla G_{A}$ 
\begin{equation}
    \begin{split}
        G_{A}\nabla G_{A} &=\begin{bmatrix}0&e^{i\chi^{*}}\\e^{-i\chi^{*}}&0\end{bmatrix}\pdv{\theta^{*}}{x}\nonumber\\&+\begin{bmatrix}i\sinh^{2}{\theta^{*}}&i\cosh{\theta^{*}}\sinh{\theta^{*}}e^{i\chi^{*}}\\-i\cosh{\theta^{*}}\sinh{\theta^{*}}e^{-i\chi^{*}}&-i\sinh^{2}{\theta^{*}}\end{bmatrix}\pdv{\chi^{*}}{x}.
    \end{split}
\end{equation}
From this it can be calculated that
\begin{equation}\label{eq:GAnablaGA}
    \begin{split}
        &\text{Tr}(G_{A}\nabla G_{A}) = 0,\\
        &\text{Tr}(\tau_{3}G_{A}\nabla G_{A}) = 2i\sinh^{2}{\theta^{*}}\pdv{\chi^{*}}{x}.
    \end{split}
\end{equation}
From equations \ref{eq:GRnablaGR} and \ref{eq:GAnablaGA} it now follows that
\begin{equation}
\begin{split}
    &\text{Tr}(G_{R}\nabla G_{R}-G_{A}\nabla G_{A}) = 0.\\
    &\text{Tr}(\tau_{3}(G_{R}\nabla G_{R}-G_{A}\nabla G_{A})) = 2i\sinh^{2}{\theta}\pdv{\chi}{x}-2i\sinh{\theta^{*}}\pdv{\chi^{*}}{x}\\& = -4\text{Im}(\sinh^{2}{\theta}\pdv{\chi}{x}).
\end{split}
\end{equation}
This latter quantity is defined as $ImIs$.
\subsubsection{Parametrised Keldysh equation}
With the expressions from the previous section \ref{eq:DLdef}, \ref{eq:CTdef}, \ref{eq:CLdef} and \ref{eq:DTdef} the Keldysh differential equation \ref{eq:Keldyshnopar} can be put in parametrised form. Taking the trace of \ref{eq:Keldyshnopar} gives
\begin{equation}\label{eq:Keldyshpar1}
    \nabla (D_{L}\nabla f_{L})+\nabla(C_{L}\nabla f_{T})+ImIs\nabla f_{T} + \text{Tr}(S) = 0.
\end{equation}
The second equation is found by taking the trace of \ref{eq:Keldyshnopar} after multiplying by $\tau_{3}$. This gives
\begin{equation}\label{eq:Keldyshpar2}
    \nabla (D_{T}\nabla f_{T})+\nabla(C_{T}\nabla f_{L})+ImIs\nabla f_{L}+ \text{Tr}(\tau_{3}S) = 0.
\end{equation}
Compared with expressions in literature \cite{belzig1999quasiclassical}, \cite{brinkman2003microscopic}, there is one extra term in each equation, $\nabla(C_{L}\nabla f_{T})$ and $\nabla(C_{T}\nabla f_{L})$. Now, these terms are proportional to $\sinh{2\text{Im}\chi}$, which means that they vanish if $\chi$ is real. Thus, in case $\chi$ is real the equations presented in \cite{belzig1999quasiclassical}, \cite{brinkman2003microscopic} are recovered.
\end{widetext}

==> OneD.tex <==
\section{The one-dimensional s + p-wave junction}
The new form of the boundary condition was used to solve the Usadel equation \cite{usadel1970generalized} for an SNN junction using mixed s + p-wave superconductors.
In this section the results of the code are discussed for the case of a one-dimensional metal, in which there is only one mode, with $\phi = 0$.
Thus, the superconductor pair potentials $\Delta_{+} = \Delta(\phi = 0)$ and $\Delta_{-}(\phi = \pi)$ for $\uparrow\downarrow$
\begin{equation}
    \Delta_{\pm} = \frac{1}{\sqrt{r^{2}+1}}\pm\frac{r}{\sqrt{r^{2}+1}},\\
\end{equation}
where $r = \frac{\Delta_{p}}{\Delta_{s}}$ is the ratio between the magnitude of the p-wave component and the s-wave component of the pair potential, as in \cite{mishra2021effects}.
In the bulk superconductor s-wave superconductivity is singlet superconductivity \cite{belzig1999quasiclassical}, whereas p-wave superconductivity is triplet superconductivity \cite{tanaka2003circuit}. The superconductor pair potential for opposite spin pairs ($\downarrow\uparrow$) is thus
\begin{equation}
    \Delta_{\pm} = -\frac{1}{\sqrt{r^{2}+1}}\pm\frac{r}{\sqrt{r^{2}+1}}.
\end{equation}
An overview of the parameters used is shown in table.
\begin{table}
    \centering
    \begin{tabular}{|l|l|}
    \hline
    Parameter     & Value \\
    \hline
         $\gamma_{B}$& 2\\
         z&1.5\\
         $E_{Th}$&0.02\\
    \hline
    \end{tabular}
    \caption{Parameters of the junction as used in the code.}
    \label{tab:my_label}
\end{table}
The density of states and pair amplitude near the superconductor-normal metal interface and the conductance of the junction were calculated for various $r$. The result for the density of states is shown in figure \ref{fig:Mixture}. It was found that at low energies there is a binary distinction, $\lim_{E\xrightarrow{}0}\rho(E)$ only depends on whether $r<1$ or $r>1$, not on the precise value of $r$. For larger energies the precise value of $r$ does make a difference, but the results are qualitatively similar in the regions $r\in(0,1)$, where the s-wave component is dominant, and $r\in(1,\infty)$, where the p-wave component is dominant, respectively. If the s-wave component is larger than the p-wave component the density of states attains a minimum at $E = 0$ and a less pronounced maximum at nonzero energy. As shown in figure \ref{fig:MixtureSP}, the energy at which this maximum is attained depends on the actual value if $\frac{\Delta_{p}}{\Delta_{s}}$. If $\frac{\Delta_{p}}{\Delta_{s}}<<1$ the peak is attained at $\frac{E}{\Delta}\approx 1$, an increase of the p-wave component shifts the maximum to lower energies. Moreover, the maximum density of states becomes considerably larger.  If the p-wave component is larger than the s-wave component however, this is reversed, there is a maximum at $E = 0$ and a less pronounced minimum at nonzero energies.  The effect of the shift of the minimum with $r$ for $r>1$ is less apparent than the shift of the maximum with $r$ for $r<1$. The effect of an increase of the depth of the dip is however visible, as it is for $r<1$. For large energies $E>>1$, the density of states is almost the same as the density of states in the normal state, both if the s-wave component is dominant and if the p-wave component is dominant.
\begin{figure}
    \centering
    \subcaptionbox{$E\in(-1.5,1.5)$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Mixture.png}}
\hfill
\subcaptionbox{ $E\in(-0.1,0.1)$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Mixturezoom.png}}
    \caption{The density of states in the normal metal at the boundary with the superconductor for different values of $r$. If the s-wave component is dominant there is a dip in the density of states, if the p-wave component is dominant the density of states peaks at zero energy. On the smaller energy scale it is clear that for low energies, only depends on which component is dominant, not on the precise value of $r$.}
    \label{fig:Mixture}
\end{figure}
\begin{figure}
    \centering
    \subcaptionbox{$r<1$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/MixtureS.png}}
\hfill
\subcaptionbox{ $E\in(-0.1,0.1)$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/MixtureP.png}}
    \caption{The density of states in the normal metal at the boundary with the superconductor at zero energy is constant in the regions $[0,1)$ and $(1,\infty]$, with a jump at $r = 1$. The density of states at $E\neq 0$ depends on the actual value of $r$.}
    \label{fig:MixtureSP}
\end{figure}


The influence of $r$ is more apparent when looking at the pairing amplitude. From the results, the pair amplitudes $F_{1} = \sinh{\theta}\cos{\chi}$ and $F_{2} = \sinh{\theta}\sin{\chi}$ can be calculated. From these quantities, the singlet amplitude $F_{1,2\uparrow}-F_{1,2\downarrow}$ and the triplet amplitude $F_{1,2\uparrow}+F_{1,2\downarrow}$ were calculated. The results are shown in figure \ref{fig:Fr}.\\
A similarity between all results is that $F_{2\uparrow}-F_{2\downarrow}$ and $F_{1\uparrow}+F_{1\downarrow}$ are always zero, whereas the other two components may be nonzero. \textcolor{red}{This can be seen from symmetry arguments, if the parity is required to be even, than only even frequency singlet and odd frequency triplet pairings can exist, no even frequency triplet or odd frequency singlet.}\textcolor{green}{Sasha, any opinion?}\\
If the superconductor used is a pure s-wave superconductor, then only a singlet component is present, if the superconductor used is a pure p-wave superconductor, then only a triplet component is present, consistent with literature. For $r\in(0,\infty)$, both components are present. For $E = 0$ only one component is non vanishing, being the singlet component if $r<1$ and the triplet component if $r>1$, but for $E>0$ both appear. As $E$ is increased, the amplitudes become more and more equal. This is more apparent if $r$ is closer to 1. This latter property can be inferred from the imaginary part of $\chi$, as detailed in supplementary material \ref{sec:nondominant}. This shows that the properties of the junction are influenced by the non-dominant component of the superconductor pair potential, but that there is a discontinuous transition from s-wave dominant to p-wave dominant superconductor junctions.
\begin{figure}
    \centering
    \subcaptionbox{$r = 0$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fr0new.png}}
\hfill
\subcaptionbox{$r = 0.2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fr0p2new.png}}
\hfill
\subcaptionbox{$r = 0.9$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fr0p9new.png}}
\hfill
\subcaptionbox{$r = 1.05$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fr1p05new.png}}
\hfill
\subcaptionbox{$r = 2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fr2new.png}}
\hfill
\subcaptionbox{$r = \infty$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/FrInfnew.png}}
    \caption{The singlet and triplet components in the normal metal for different values of $r$. The gauge was chosen such that $F_{1}$ corresponds to bulk s-wave superconductors. Only two components, singlet $F_{1}$ and triplet $F_{2}$ can be nonzero. If $r<1$ the singlet component is dominant, if $r>1$ the triplet component is dominant. At low energies the behaviour is very similar to pure type superconductors, for higher energies the components are much more similar. If $r$ is closer to one the components are more similar.}
    \label{fig:Fr}
\end{figure}
The third quantity of interest is the conductance, defined by
\begin{align}
    \sigma &= R^{-1},\\
    %R &= \frac{1}{2}\left(\frac{R_{B}}{I_{b0}}+\frac{R_{d}}{L}\int_{0}^{L}\frac{dx}{1+|\cosh{\theta}|^{2}+|\sinh{\theta}|^{2}\cosh{\text{Im}\chi}}\right).
    R&= \frac{1}{2}(1+X_{3}\frac{I_{b1}}{I_{b0}})^{-1}\left(\frac{R_{b}}{I_{b0}}+\frac{R_{d}}{L}X_{4}\right),
\end{align}
where
\begin{align}
    X_{3}& =\left(1+\frac{I_{b2}}{\gamma_{B}L}\int_{0}^{L}\frac{1}{D_{L}+\frac{C^{2}}{D_{T}}}dx-\frac{I_{b1}}{\gamma_{B}L}\int_{0}^{L}\frac{C}{D_{L}D_{T}+C^{2}}dx\right)^{-1}\nonumber\\&\left(-\frac{I_{b3}}{\gamma_{B}L}\int_{0}^{L}\frac{1}{D_{L}+\frac{C^{2}}{D_{T}}}dx+\frac{I_{b0}}{\gamma_{B}L}\int_{0}^{L}\frac{C}{D_{L}D_{T}+C^{2}}dx\right),\\
    X_{4}& =\int_{0}^{L}\frac{1}{D_{T}+\frac{C^{2}}{D_{L}}}dx+\frac{I_{b3}}{I_{b0}}\int_{0}^{L}\frac{C}{D_{L}D_{T}+C^{2}}dx+X_{3}\left(\frac{I_{b1}}{I_{b0}}\int_{0}^{L}\frac{1}{D_{T}+\frac{C^{2}}{D_{L}}}dx+\frac{I_{b2}}{I_{b0}}\int_{0}^{L}\frac{C}{D_{L}D_{T}+C^{2}}dx\right),\\
    D_{L} & = D_{L\uparrow,
    } &= 1+|\cosh{\theta_{\uparrow,
    }}|^{2}-|\sinh{\theta_{\uparrow,
    }}|^{2}\cosh{2\text{Im}(\chi_{\uparrow,
    })}\\
    D_{T} & =1+|\cosh{\theta_{\uparrow,
    }}|^{2}+|\sinh{\theta_{\uparrow,
    }}|^{2}\cosh{2\text{Im}(\chi_{\uparrow,
    })} \\
    C &=  -|\sinh{\theta_{\uparrow,
    }} |^{2}\sinh{2\text{Im}(\chi_{\uparrow,
    })},
\end{align}
where $I_{b0}, I_{b1},I_{b2},I_{b3}$ follow from the Tanaka-Nazarov boundary condition. A discussion of these quantities and a derivation of $R$ can be found in supplementary material \ref{sec:NEWconductanceformula}.
Here $\theta$ and $\chi$ are the parameters from the retarded equation, which are known. The quantity $I_{b0}$ comes from the Tanaka-Nazarov boundary condition. An expression for this quantity and a discussion of the derivation is given in supplementary material \ref{sec:NEWconductanceformula}.
The results, normalised to $R_{b}+R_{d}$, are shown in figure \ref{fig:Sigmarplot}. There is a clear correspondence between the results for the density of states and for the conductance in that the low energy behaviour is completely determined by the dominant component in the superconductor. If the p-wave component is dominant there is a zero bias conductance peak, which magnitude is almost independent of $r$, if the s-wave component is dominant this zero bias conductance peak is absent. The behaviour of $\sigma$ around $eV = \Delta$ however, is greatly influenced by the exact value of $r$. For each $r$ the conductance has different behaviour in three distinct regions, with almost discontinuous derivatives at $eV = \Delta_{\pm}$. For s-wave dominant superconductor junctions, the conductance is almost constant between $eV = \Delta_{\pm} = \frac{1\pm r}{\sqrt{1+r^{2}}}$, this plateau being a maximum of the conductance. For p-wave dominant superconductor junctions the conductance decreases as a function of $V$ up to $eV\approx|\Delta_{-}|$, and then increases in the region $eV \in(|\Delta_{-}|, \Delta_{+})$. For all $r$, it was found that for $eV>\Delta_{+}$ the conductance monotonically approaches $\sigma = 1$, that is, at large voltages $eV>>\Delta_{+}$, the normal metal resistance is attained regardless of $r$, as expected.
\begin{figure}
    \centering
    \includegraphics[width = 0.7\textwidth]{figures/Sigmarplot1new26.png}
    \caption{The conductance $\sigma$ of the junction for different values of $r$. If the p-wave component is dominant there is a zero-bias conductance peak, which is absent if the s-wave component is dominant. For this single channel model the height of the zero bias conductance peak is independent of $r$ for $r>1$.}
    \label{fig:Sigmarplot}
\end{figure}
\begin{figure}
    \centering
    \subcaptionbox{$r = 0$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/SigmaeVR1D.png}}
\hfill
\subcaptionbox{$r = 0.2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/SigmaeV01D.png}}

    \caption{The conduction in the 1D SNN junction as a function of voltage and $\frac{r}{1+r}$. The distinction between the two cases is clearly visible. For $r<1$ there is a dip in the density of states at low energies, for $r>1$ there is a peak at low energies. The width of the peak or dip decreases as the contributions from the s-wave and p-wave component become more equal in strength. There is discontinuous change of the conductance at zero voltage at $r = 1$, that is $\frac{r}{1+r} = \frac{1}{2}$.}
    \label{fig:SigmaeV1D}
\end{figure}
\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsection{Length of the junction}
The influence of the length of the junction was studied by increasing and decreasing the length by a factor 2. This is equivalent to decreasing and increasing the Thouless energy by a factor 4. The results found are shown in figure \ref{fig:FrL}. It was found that the results at $E = 0$ are independent of the length of the junction. This can be explained analytically as well, as for $E = 0$ the solution to the Usadel equation is linear, with $\dv{\theta}{x}\propto\frac{1}{L}$ and hence $\theta(0) = -\int_{0}^{L}\dv{\theta}{x} = \theta_{0}$ is independent of the length of the junction. Thus, the zero energy Green's function is independent of the length of the junction. For $E>0$ however, the length of the junction does have an influence. If the Thouless energy is increased, the peak of the pair amplitude at zero energy becomes much broader. In general, if $E_{Th}$ is increased, then also $F(E>0)$ increases. This means that for larger $E_{Th}$ the non-dominant component, which vanishes for $E = 0$ but not for $E>0$, is more apparent. As expected, in- or decreasing the Thouless energy has no influence on the two components that absent in the junction. The results for the conductance show a very similar difference. The height of the zero bias conductance peak is independent of the length of the junction, however, its width is greatly influenced by it.
\begin{figure}
    \centering
    \subcaptionbox{$r = 0.2$, $E_{Th} = 0.005$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fr0p2t2new.png}}
\hfill
\subcaptionbox{$r = 0.2$, $E_{Th} = 0.08$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fr0p2d2new.png}}
\hfill
\subcaptionbox{$r = 1.05$, $E_{Th} = 0.005$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fr1p05t2new.png}}
\hfill
\subcaptionbox{$r = 1.05$, $E_{Th} = 0.08$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fr1p05d2new.png}}
\hfill
    \caption{The singlet and triplet components in the normal metal for different values of $r$ and $E_{Th}$. One singlet dominant and one triplet dominant junction are shown. The gauge was chosen such that $F_{1}$ corresponds to bulk s-wave superconductors. The $r$-dependence of the pair amplitude remains very similar, if the s-wave (p-wave) component is dominant, then the singlet (triplet) pair amplitude is larger over the whole energy range, with the difference being most apparent at low energies. If the Thouless energy is increased, the pair amplitude is larger in the higher energy regime, near zero energy the pair amplitude is independent of the length of the junction. Because the pair amplitude is larger for larger energies the non-dominant amplitude appears more clearly if the Thouless energy is increased. This holds both if the singlet component is dominant and if the triplet component is dominant.}
    \label{fig:FrL}
\end{figure}
Also the conductance remains qualitatively the same if the Thouless energy is increased or decreased, as shown in figure \ref{fig:SigmaRL}. In correspondence with the pair amplitude, if the Thouless energy is decreased, the zero bias conductance peak for p-wave dominant superconductor junctions becomes sharper. This is detailed further in figure \ref{fig:SigmaL}. For low energies (but $(E>0)$) the results for different Thouless energies are different, but at $E = 0$ and for $E>>E_{Th}$ the results are very similar.
\begin{figure}
    \centering
    \subcaptionbox{$E_{Th} = 0.005$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/SigmarLt2new26.png}}
\hfill
\subcaptionbox{$E_{Th} = 0.08$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/SigmarLd2new26.png}}
    \caption{The conductance in the junction for different values of $r$ when the length of the junction is doubled and when the length of the junction is halved. I the Thouless energy is smaller the zero bias conductance peak becomes narrower, but its height remains the same, in correspondence with analytical considerations. The high energy conductance has a much smaller length dependence.}
    \label{fig:SigmaRL}
\end{figure}
\begin{figure}
    \centering
    \subcaptionbox{$r = 0$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/sigmar0L26.png}}
\hfill
\subcaptionbox{$r =2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Sigmar2L26.png}}
    \caption{Comparison of the conductance in the junction when the length of the junction is varied. Both a singlet dominant $(r<1)$ and a triplet dominant $(r>1)$ are shown. The magnitude of the Thouless energy has its main influence for low voltages, where the voltage dependence of the differential conductance is stronger if the Thouless energy is smaller. In the large voltage regime the results are very similar if $L$ is varied.}
    \label{fig:SigmaL}
\end{figure}
\newpage
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}

\subsection{Boundary resistance}
In the previous section it was confirmed that the length of the junction has no influence on the solution at $E = 0$. A quantity that should influence the result at $E = 0$ is $\gamma_{B}$, since $\dv{\theta}{x}\propto\frac{1}{\gamma_{B}}$, and hence $\theta(0) = -\int_{0}^{L}\dv{\theta}{x}dx\propto\frac{1}{\gamma_{B}}$. To test this, the calculations were repeated for an increase of $\gamma_{B}$ by a factor of 2 and for a decrease of $\gamma_{B}$ by a factor of 2. The newly computed pair amplitudes are shown in figure \ref{fig:FrG}. As expected, an increase of $\gamma_{B}$ leads to a suppression of the pair amplitude, whereas for a decrease of $\gamma_{B}$ the pair amplitude becomes much larger. The variation of $\gamma_{B}$ causes no clear differences in the dominance of triplet or singlet pair amplitudes, except at very low energies, where the larger peak at zero energy means that the dominant pair amplitude is more favoured for smaller $\gamma_{B}$.
\begin{figure}
    \centering
    \subcaptionbox{$r = 0.2$, $\gamma_{B} = 4$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fr0p2gt2new.png}}
\hfill
\subcaptionbox{$r = 0.2$, $\gamma_{B} = 1$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fr0p2gd2new.png}}
\hfill
\subcaptionbox{$r = 1.05$, $\gamma_{B} = 4$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fr1p05gt2new.png}}
\hfill
\subcaptionbox{$r = 1.05$, $\gamma_{B} = 1$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Fr1p05gd2new.png}}
\hfill
    \caption{The singlet and triplet components in the normal metal for different values of $r$ and $\gamma_{B}$. One singlet dominant and one triplet dominant junction are shown. The gauge was chosen such that $F_{1}$ corresponds to bulk s-wave superconductors.The $r$-dependence of the pair amplitude remains very similar, if the s-wave (p-wave) component is dominant, then the singlet (triplet) pair amplitude is larger over the whole energy range, with the difference being most apparent at low energies. If the boundary resistance is increased relative to $R_{d}$, the pair amplitude becomes more suppressed. This effect is stronger if the p-wave component is dominant, the height of the peak at zero energy depends strongly on $\gamma_{B}$.}
    \label{fig:FrG}
\end{figure}
There is also a clear increase in the conductance of the junction if $\gamma_{B}$ is lowered, although the variation is less extreme compared to the difference in pair amplitude. For s-wave dominant junctions, a larger $\gamma_{B}$ suppresses the conductance peak around $eV = \Delta$, for p-wave dominant junctions the height of the zero bias conductance peak is lowered. The results for $\sigma(eV = 0)$ have been calculated analytically for the one-dimensional junction in WHAT TO CITE. The results is
\begin{equation}
    \sigma(eV = 0) = \frac{1+\frac{R_{b}}{R_{d}}}{\frac{R_{b}}{R_{d}}\langle T\rangle}.
\end{equation}
The results as shown in figure \ref{fig:SigmaRG} are consistent with this calculation.
\begin{figure}
    \centering
    \subcaptionbox{$\gamma_{B} = 4$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Sigmargt2new26.png}}
\hfill
\subcaptionbox{$\gamma_{B} = 2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Sigmargd2new26.png}}
    \caption{The conductance in the junction for different values of $r$ when the boundary resistance is doubled or halved. The dependence of the conductance on $r$ remains similar. However, if the boundary resistance is increased, the zero bias conductance peak is much more suppressed and the conductance is closer to 1.}
    \label{fig:SigmaRG}
\end{figure}
\begin{figure}
    \centering
    \subcaptionbox{$r = 0$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Sigmar0G26.png}}
\hfill
\subcaptionbox{$r =2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Sigmar2G26.png}}
    \caption{Comparison of the conductance in the junction if the boundary resistance is increased. For the singlet dominant case the peak around $eV = \Delta$ is suppressed if the boundary resistance is increased, for the triplet dominant case the height of the zero bias conductance peak changes if the boundary resistance is increased. The effect for $r>1$ is larger than for $r<1$.}
    \label{fig:SigmaG}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\end{comment}

\subsection{The tipping point, r = 1}
The tipping point is at $r = 1$, where the s-wave and p-wave contributions are equal. In that case $\Delta_{+} = \Delta_{s}+\Delta_{p} = 2\Delta_{s}$ and $\Delta_{-} = \Delta_{s}-\Delta_{p} = 0$. This means that $g_{m} = 1$ and $f_{m} = 0$. Due to this, the parameter $\chi$ becomes undetermined, because the denominator within the logarithm vanishes.
However, $C$ can be calculated explicitly.
\begin{align}
    R_{m} &= \frac{1}{2}\begin{bmatrix}g_{p}-1&f_{p}e^{i\psi}\\-f_{p}e^{-i\psi}&-g_{p}+1\end{bmatrix},\\
    R_{p} &= \frac{1}{2}\begin{bmatrix}g_{p}+1&f_{p}e^{i\psi}\\-f_{p}e^{-i\psi}&-g_{p}-1\end{bmatrix},\\
    R_{p}^{-1} &= \frac{1}{1+g_{p}}\begin{bmatrix}g_{p}+1&f_{p}e^{i\psi}\\-f_{p}e^{-i\psi}&-g_{p}-1\end{bmatrix},\\
    R_{p}^{-1}R_{m} &= \frac{1}{2(1+g_{p})}\begin{bmatrix}g_{p}^{2}-1-f_{p}^{2}&g_{p}f_{p}e^{i\psi}+f_{p}e^{i\psi}-g_{p}f_{p}e^{i\psi}+f_{p}e^{i\psi}\\-g_{p}f_{p}e^{-i\psi}+f_{p}e^{-i\psi}+g_{p}f_{p}e^{-i\psi}+f_{p}e^{-i\psi}&g_{p}^{2}-1-f_{p}^{2}\end{bmatrix}\nonumber\\
    &=\frac{1}{1+g_{p}}\begin{bmatrix}0&f_{p}e^{i\psi}\\f_{p}e^{-i\psi}&0\end{bmatrix},\\
    C &= R_{p}^{-1}-R_{p}^{-1}R_{m} = \begin{bmatrix}1&0\\-\frac{2f_{p}}{1+g_{p}}&-1\end{bmatrix}.
\end{align}
This last line shows that $C$ is not within the range of matrices that can be described by the $\theta$-parametrisation. Based on this, the following Ansatz can be used for the solution of the equation:
\begin{equation}
    G(x) = \begin{bmatrix}1&0\\g(x)&-1\end{bmatrix}.
\end{equation}
Notice that $G(x)^2 = \mathbf{1}$ is automatically satisfied.

It can be calculated that in that case
\begin{align}
    G\nabla G = \begin{bmatrix}0&0\\-\nabla g&0\end{bmatrix},
    [\tau_{3},G] = -2\begin{bmatrix}0&0\\g&0\end{bmatrix}.
\end{align}
Thus, the Usadel equation reduces to the linear equation
\begin{equation}
    \nabla^{2}g+2iEg = 0.
\end{equation}
Moreover,
\begin{align}
    CG-GC &= 2\begin{bmatrix}0&0\\-\frac{2f_{p}}{1+g_{p}}-g&0\end{bmatrix},\\
    CG+GC &=2\begin{bmatrix}1&0\\0&1\end{bmatrix},
\end{align}
which means that 
\begin{align}
    I = S(G) = 2T((4-2T)\mathbf{1}+T(CG+GC))^{1}(CG-GC) = T\begin{bmatrix}0&0\\-\frac{2f_{p}}{1+g_{p}}-g&0\end{bmatrix}.
\end{align}
Thus, the parametrisation is also consistent with the boundary condition $G\nabla G = \frac{1}{\gamma_{B}LT}I$, giving the system
\begin{align}
    &\nabla^{2}g+2iEg = 0,\\
    &\nabla g (x = 0)  = -\frac{T}{\gamma_{B}LT}(-\frac{2f_{p}}{1+g_{p}}-g)\\
    &g\to 0 \text{as} x\to\infty,
\end{align}
where the last condition indicates that the normal metal state should be approached far away from the interface. This is a linear equation, which can be solved to give
\begin{equation}
    g(x) = \left(\frac{T}{\gamma_{B}LT}+\sqrt{E}(1-i)\right)^{-1}2\frac{T}{\gamma_{B}LT}\frac{f_{p}}{1+g_{p}}e^{-\sqrt{E}(1-i)x}.
\end{equation}
This is the solution for $r = 1$. The density of states of the normal metal is not altered, but there is a proximity effect as $g\neq 0$.\\
For a finite junction, the condition $g\to0$ as $x\to\infty$ is replaced by $g(L) = 0$. In that case 
\begin{equation}
    g(x) = -\left(\frac{T}{\gamma_{B}LT}+\sqrt{E}(1-i)\big(1-e^{-2\sqrt{E}(1-i)L}\big)\right)^{-1}2\frac{T}{\gamma_{B}LT}\frac{f_{p}}{1+g_{p}}\left(e^{-\sqrt{E}(1-i)x}-e^{\sqrt{E}(1-i)(x-2L)}\right).
\end{equation}
This expression is very similar to the case of an infinite wire.
\subsubsection{Opposite spin}
For the opposite spin, it holds that $\Delta_{+} = 0$ and $\Delta_{-} = -2\Delta_{s}$. Therefore, in this case, $g_{p} = 1$ and $f_{p} = 0$, whereas $g_{m\downarrow} = g_{p\uparrow}$ and $f_{m\downarrow} = -f_{p\uparrow}$, where the notation $\uparrow$ refers to the previously calculated spin component, and $\downarrow$ to the spin component that will be discussed in this section.
Therefore in this case, omitting $\downarrow$ for simplicity of notation
\begin{align}
    R_{m} &= \frac{1}{2}\begin{bmatrix}1-g_{m}&-f_{m}e^{i\psi}\\f_{m}e^{-i\psi}&-1+g_{m}\end{bmatrix},\\
    R_{p} &= \frac{1}{2}\begin{bmatrix}g_{m}+1&f_{m}e^{i\psi}\\-f_{m}e^{-i\psi}&-g_{m}-1\end{bmatrix},\\
    R_{p}^{-1} &= \frac{1}{1+g_{m}}\begin{bmatrix}g_{m}+1&f_{m}e^{i\psi}\\-f_{m}e^{-i\psi}&-g_{m}-1\end{bmatrix},\\
    R_{p}^{-1}R_{m} &=
    %\frac{1}{2(1+g_{m})}\begin{bmatrix}-g_{m}^{2}+1+f_{m}^{2}&-g_{m}f_{m}e^{i\psi}-f_{m}e^{i\psi}+g_{m}f_{m}e^{i\psi}-f_{m}e^{i\psi}\\g_{m}f_{m}e^{-i\psi}-f_{m}e^{-i\psi}-g_{m}f_{m}e^{-i\psi}-f_{m}e^{-i\psi}&-g_{m}^{2}+1+f_{m}^{2}\end{bmatrix}\nonumber\\
    %&=
    \frac{1}{1+g_{m}}\begin{bmatrix}0&-f_{m}e^{i\psi}\\-f_{m}e^{-i\psi}&0\end{bmatrix},\\
    C &= R_{p}^{-1}-R_{p}^{-1}R_{m} = \begin{bmatrix}1&\frac{2f_{m}}{1+g_{m}}\\0&-1\end{bmatrix}.
\end{align}
Thus,
\begin{equation}
    G_{\downarrow}(x) = \begin{bmatrix}1&g_{\downarrow}(x)\\0&-1\end{bmatrix},
\end{equation}
which satisfies $G_{\downarrow}^2 = 1$. In this case
\begin{equation}
    G_{\downarrow}\nabla G_{\downarrow} = \begin{bmatrix}0&\nabla g_{\downarrow}\\0&0\end{bmatrix}, [\tau_{3},G] = 2\begin{bmatrix}0&g_{\downarrow}\\0&0\end{bmatrix},
\end{equation}
and therefore the Usadel equation reduces to the same equation as for the spin up component,
\begin{equation}
    \nabla^{2}g_{\downarrow}+2iEg_{\downarrow} = 0.
\end{equation}
For the boundary condition, notice that
\begin{align}
    CG-GC = 2\begin{bmatrix}0&g_{\downarrow}-2\frac{f_{m}}{1+g_{m}}\\0&0\end{bmatrix},
    CG+GC = 2\begin{bmatrix}1&0\\0&1\end{bmatrix},
\end{align}
which means that
\begin{align}
    I &= S(G) = 2\sigma((4-2\sigma)\mathbf{1}+\sigma(CG+GC))^{1}(CG-GC) = \sigma\begin{bmatrix}0&g_{\downarrow}-2\frac{f_{m}}{1+g_{m}}\\0&0\end{bmatrix}.\\
    & =2\sigma((4-2\sigma)\mathbf{1}+\sigma(CG+GC))^{1}(CG-GC) = \sigma\begin{bmatrix}0&g_{\downarrow}+2\frac{f_{p\uparrow}}{1+g_{p\uparrow}}\\0&0\end{bmatrix} .
\end{align}
Thus, also the boundary condition for $g_{\downarrow}$ is the same as for $g_{\uparrow}$. Therefore, it can be concluded that 
\begin{equation}
g_{\uparrow} = g_{\downarrow} = g = C\left(e^{-\sqrt{E}(1-i)x}-e^{\sqrt{E}(1-i)(x-2L)}\right),
\end{equation}
where
\begin{equation}
    C = -\left(\frac{T}{\gamma_{B}LT}+\sqrt{E}(1-i)\big(1-e^{-2\sqrt{E}(1-i)L}\big)\right)^{-1}2\frac{T}{\gamma_{B}LT}\frac{f_{p}}{1+g_{p}}.
\end{equation}
\subsubsection{Conductance}
Also the conductance can be calculated for $r = 1$. Recall that the conductance is given by $\sigma = R^{-1}$, where \cite{tanaka2021phys}:
\begin{equation}
    R = \frac{1}{2}\left(\frac{R_{b}}{I_{B0}}+\frac{R_{d}}{L}\int_{0}^{L}\frac{dx}{F(g)} \right),
\end{equation}
where
\begin{align}
    F(g) &= \frac{1}{2}(1+|s_{1}|^{2}+|s_{2}|^{2}+|s_{3}|^{2}).
\end{align}
For $r = 1$, it holds that
\begin{align}
    F(g) &= \frac{1}{2}(1+|s_{1}|^{2}+|s_{2}|^{2}+|s_{3}|^{2}) = 1+\frac{1}{4}|g(x)|^2\\& = 1+\frac{|C|^{2}}{4}(e^{-2\sqrt{E}x}+e^{2\sqrt{E}(x-2L)}-2e^{-2\sqrt{E}L}\cos{2\sqrt{E}(x-L)})\nonumber\\&=1+\frac{|C|^{2}}{2}e^{-2\sqrt{E}L}\left(\cosh{2\sqrt{E}(x-L)}-\cos{2\sqrt{E}(x-L)}\right).
\end{align}
Moreover, recall that
\begin{align}
    I_{b0} &= \frac{T_{1}}{2T|d_{R}|^{2}}e_{R},\\
    & e_{R}= \text{Tr}\left((R+R^{\dagger})(C+C^{\dagger})(1+T_{1}^{2})+2T_{1}(1+RR^{\dagger})(1+CC^{\dagger})\right),\\
    d_{R} &=\frac{1}{2}\text{Tr}(1+T_{1}^{2}+2T_{1}(CG+GC)).
\end{align}
Now, for $r = 1$
\begin{align}
    e_{R} &= (1+T_{1})^{2}\left(8-\text{Re}(g(0)\frac{2f_{p}}{1+g_{p}})\right)+2T_{1}\left(8+2\big(|g(0)|^{2}+|\frac{2f_{p}}{1+g_{p}}|^{2}+\text{Re}(g(0)\frac{2f_{p}}{1+g_{p}})\big)\right)\\
    d_{R}& = (1+T_{1})^{2}.
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Px.tex <==
\section{Twodimensional junctions}
In \cite{tanaka2021phys} a new form of the Tanaka-Nazarov boundary condition was derived, and this new form was used to study one-dimensional SN junctions. Next to the purely one-dimensional bar, also a two dimensional bar in which the Green's function has no y-dependence can be considered, that is, either a bar that is thin enough that the one-dimensional Usadel equation can be studied, for which multiple modes contribute to the Tanaka-Nazarov conditions \cite{nazarov1999novel} \cite{tanaka2003circuit}, \cite{tanaka2004theory}, or a very wide junction, so that boundaries are far away. In this case, the Usadel equation does not change, but in the boundary condition several modes should be used. The modes are integrated as specified in \cite{tanaka2004theory}. For pairs with opposite spin, the s-wave potential changes sign, whereas the p-wave potential does not. As this work is an extension of \cite{tanaka2021phys}, the same parameters in the Tanaka-Nazarov boundary condition, that is, the ratio between boundary resistance and bar resistance is $\gamma_{B} = 2$, transparency is given by $T = \frac{\cos^{2}{\phi}}{\cos^{2}{\phi}+z^{2}}$ with $z = 1.5$ and a Thouless energy $E_{Th} = 0.02\Delta$ were used. 
The density of states and pair amplitude near the superconductor-normal metal interface and the conductance of the junction were calculated for various $r$. The pair amplitudes $F_{1} = \sinh{\theta}\cos{\chi}$ and $F_{2} = \sinh{\theta}\sin{\chi}$ were be calculated. From these quantities, the singlet amplitude $F_{1,2\uparrow}-F_{1,2\downarrow}$ and the triplet amplitude $F_{1,2\uparrow}+F_{1,2\downarrow}$ were calculated.\\
A similarity between all results is that $F_{2\uparrow}-F_{2\downarrow}$ and $F_{1\uparrow}+F_{1\downarrow}$ are always zero, whereas the other two components may be nonzero. \textcolor{red}{This can be seen from symmetry arguments, if the parity is required to be even, than only even frequency singlet and odd frequency triplet pairings can exist, no even frequency triplet or odd frequency singlet.}\textcolor{green}{Sasha, any opinion?}\\
\section{Twodimensional $\text{p}_{\text{x}}$-wave junction}
The superconductor pair potential of a 2D s + $\text{p}_{\text{x}}$-wave superconductor is, \begin{equation}\label{eq:s+p2D}
    \Delta_{\pm} = \frac{1}{\sqrt{r^{2}+1}}\pm\frac{r}{\sqrt{r^{2}+1}}\cos{\phi-\phi_{m}},
\end{equation}
where $\phi$ is the angle of the mode with the normal, and $\phi_{m}$ is the angle that the mode with maximum $\Delta_{+}$ makes with the surface normal. In this work $\phi_{m} = 0$, unless otherwise specified. \\
The density of states, pair amplitude and conductance were calculated for the same parameter set as for the one-dimensional junction. Similar to the one-dimensional case, there is a peak in the density of states if $r>1$ and a dip in the density of states if $r<1$. However, the behaviour at low energies is different for the quasi-one-dimensional junction than for the one-dimensional junction. Whereas for $r<1$ the magnitude of the tip is independent of $r$ as in the one-dimensional case, for $r>1$ the magnitude of the peak in the density of states depends on the value of $r$. This can be understood from equation \ref{eq:s+p2D}. If $r>1$, then $\frac{r}{\sqrt{r^{2}+1}}>\frac{1}{\sqrt{r^{2}+1}}$. Thus, at $\phi = 0$, $\Delta_{-}(0)<0$. This mode will thus always contribute to a peak in the density of states. However, if $\cos{\phi}<\frac{1}{r}$, it follows that $\Delta_{-}(\phi)>0$, and the mode will not contribute to the peak in the density of states anymore. Thus, for $r\in(1,\infty)$, only a proportion of the modes will contribute to the formation of the zero energy peak in the density of states, and this proportion increases if $r$ increases. Therefore the magnitude of the peak in the density of states depends on the value of $r$. On the other hand, if $r<1$, $\frac{r}{\sqrt{r^{2}+1}}>\frac{1}{\sqrt{r^{2}+1}}$ and therefore $\Delta_{-}(\phi)>0$ for all angles. Thus, the magnitude of the dip in the density of states is independent of $r$ if the s-wave component is dominant.
\begin{figure}
    \centering
    \includegraphics[width = 0.7\textwidth]{figures/Rhozoom.png}
    \caption{The density of states in the quasi-one-dimensional junction near the superconductor-normal metal interface. Similar to the one-dimensional junction, there is a clear peak if the p-wave component is dominant, whereas this peak is absent if the s-wave component is dominant.}
    \label{fig:Rho2D}
\end{figure}
\begin{comment}
\begin{figure}
    \centering
    \subcaptionbox{$r<1$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/rho2DSfull.png}}
\hfill
\subcaptionbox{$r>1$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/rho2DP.png}}
    \caption{The low energy density of states in the quasi-one-dimensional junction near the superconductor-normal metal interface when the s-wave component is dominant and when the p-wave component is dominant. If the s-wave component is dominant, the low energy behaviour is independent of $r$. However, if the p-wave component is dominant, the magnitude of the peak in the density of states strongly depends on $r$.}
    \label{fig:Rho2Dzoom}
\end{figure}
\end{comment}
Also the pair amplitude was investigated in the quasi-one-dimensional case. The results are shown in figure \ref{fig:Fr2D}. As for the local density of states, the results are similar to the purely one-dimensional junction \cite{tanaka2021phys}, but there are subtle differences that arise for $r>1$. If the superconductor used is a pure s-wave superconductor, then only a singlet component is present, if the superconductor used is a pure p-wave superconductor, then only a triplet component is present, consistent with literature. For $r\in(0,\infty)$, both components are present. Whereas for the purely one-dimensional junction the non-dominant component always vanishes at $E = 0$, for the quasi-one-dimensional junction this only holds for $r<1$. For $r>1$ on the other hand, the non-dominant component is non-vanishing at zero energy. 
\begin{figure}
    \centering
\subcaptionbox{$r = 0.2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/F2Dr0p2.png}}
\hfill
\subcaptionbox{$r = 2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/F2Dr2.png}}
    \caption{The singlet and triplet components in the normal metal for different values of $r$ for the quasi-one-dimensional junctions. The gauge was chosen such that $F_{1}$ corresponds to bulk s-wave superconductors. Only two components, singlet $F_{1}$ and triplet $F_{2}$ can be nonzero. If $r<1$ the singlet component is dominant, if $r>1$ the triplet component is dominant. For $r<1$ the triplet component vanishes completely as $E\xrightarrow{} 0$, however, for $r>1$ the cancellation is not complete.}
    \label{fig:Fr2D}
\end{figure}
\begin{comment}
\begin{figure}
    \centering
    \subcaptionbox{$r = 0$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/F2Dr0.png}}
\hfill
\subcaptionbox{$r = 0.2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/F2Dr0p2.png}}
\hfill
\subcaptionbox{$r = 0.9$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/F2Dr0p9.png}}
\hfill
\subcaptionbox{$r = 2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/F2Dr2.png}}
\hfill
\subcaptionbox{$r = 5$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/F2Dr5.png}}
\hfill
\subcaptionbox{$r = \infty$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/F2DrInf.png}}
    \caption{The singlet and triplet components in the normal metal for different values of $r$ for the quasi-one-dimensional junctions. The gauge was chosen such that $F_{1}$ corresponds to bulk s-wave superconductors. Only two components, singlet $F_{1}$ and triplet $F_{2}$ can be nonzero. If $r<1$ the singlet component is dominant, if $r>1$ the triplet component is dominant. For $r<1$ the triplet component vanishes completely as $E\xrightarrow{} 0$, however, for $r>1$ the cancellation is not complete.}
    \label{fig:Fr2D}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width = 0.7\textwidth]{figures/FND.png}
    \caption{The non-dominant component $F_{ND}$ at zero energy as a function of $r$. If the s-wave component of $\Delta$ is dominant there the triplet component vanishes at zero energy, if the p-wave component of $\Delta$ is dominant the singlet component does not vanish at zero energy, contrary to the one-dimensional case. As $r$ increases, $F_{ND}$ decreases towards 0.}
    \label{fig:FND}
\end{figure}
\end{comment}
The third quantity of interest is the conductance. The conductance has been calculated from the Keldysh component of the Usadel equation. Because a mixed s+p-wave superconductor was investigated, the distribution functions were specifically allowed to depend on spin, in contrast with previous works \textcolor{red}{Question to Tanaka: What paper would you like to be cited here?}. It was shown that in the case of a pure type potential, that is, s-wave or p-wave, the expressions reduce to those in \textcolor{red}{Same citation}.  A discussion of these quantities and a derivation of $R$ can be found in supplementary material \ref{sec:NEWconductanceformula}, the resulting expression is
\begin{align}
    \sigma &= R^{-1},\\
    %R &= \frac{1}{2}\left(\frac{R_{B}}{I_{b0}}+\frac{R_{d}}{L}\int_{0}^{L}\frac{dx}{1+|\cosh{\theta}|^{2}+|\sinh{\theta}|^{2}\cosh{\text{Im}\chi}}\right).
    R&= \frac{1}{2}(1+X_{3}\frac{I_{b1}}{I_{b0}})^{-1}\left(\frac{R_{b}}{I_{b0}}+\frac{R_{d}}{L}X_{4}\right),
\end{align}
where
\begin{align}
    X_{3}& =\left(1+\frac{I_{b2}}{\gamma_{B}L}\int_{0}^{L}\frac{1}{D_{L}+\frac{C^{2}}{D_{T}}}dx-\frac{I_{b1}}{\gamma_{B}L}\int_{0}^{L}\frac{C}{D_{L}D_{T}+C^{2}}dx\right)^{-1}\nonumber\\&\left(-\frac{I_{b3}}{\gamma_{B}L}\int_{0}^{L}\frac{1}{D_{L}+\frac{C^{2}}{D_{T}}}dx+\frac{I_{b0}}{\gamma_{B}L}\int_{0}^{L}\frac{C}{D_{L}D_{T}+C^{2}}dx\right),\\
    X_{4}& =\int_{0}^{L}\frac{1}{D_{T}+\frac{C^{2}}{D_{L}}}dx+\frac{I_{b3}}{I_{b0}}\int_{0}^{L}\frac{C}{D_{L}D_{T}+C^{2}}dx+X_{3}\left(\frac{I_{b1}}{I_{b0}}\int_{0}^{L}\frac{1}{D_{T}+\frac{C^{2}}{D_{L}}}dx+\frac{I_{b2}}{I_{b0}}\int_{0}^{L}\frac{C}{D_{L}D_{T}+C^{2}}dx\right),\\
    D_{L} & = D_{L\uparrow,
    } &= 1+|\cosh{\theta_{\uparrow,
    }}|^{2}-|\sinh{\theta_{\uparrow,
    }}|^{2}\cosh{2\text{Im}(\chi_{\uparrow,
    })}\\
    D_{T} & =1+|\cosh{\theta_{\uparrow,
    }}|^{2}+|\sinh{\theta_{\uparrow,
    }}|^{2}\cosh{2\text{Im}(\chi_{\uparrow,
    })} \\
    C &=  -|\sinh{\theta_{\uparrow,
    }} |^{2}\sinh{2\text{Im}(\chi_{\uparrow,
    })},
\end{align}
where $I_{b0}, I_{b1},I_{b2},I_{b3}$ follow from the Tanaka-Nazarov boundary condition.
Here $\theta$ and $\chi$ are the parameters from the retarded equation, which are known. The quantity $I_{b0}$ comes from the Tanaka-Nazarov boundary condition. An expression for this quantity and a discussion of the derivation is given in supplementary material \ref{sec:NEWconductanceformula}.
 The results are shown in figures \ref{fig:Sigma2D} and \ref{fig:SigmaeV$\text{p}_{\text{x}}$}. The results are in correspondence with the earlier obtained results, the zero bias conductance peak is only present if $r>1$ and contrary to the one-dimensional case, the height of the zero bias conductance peak depends on the value of $r$ used. For $r<1$ the zero bias conductance is constant, but for $r>1$ the zero bias conductance increases with $r$. This is contrary to the one-dimensional junction, where the zero bias conductance is constant both for $r<1$ and $r>1$, with a discontinuity at $r = 1$. In the quasi-one-dimensional junction on the other hand there is no discontinuity in the zero bias conductance, however, there is a kink, that is, a discontinuity in the derivative at $r = 1$, as shown in figure \ref{fig:SigmaeV$\text{p}_{\text{x}}$}. Another difference with the one-dimensional junction is that the conductance as a function of $V$ is smooth for the quasi-one-dimensional junction, the kinks at $eV = \Delta_{\pm}$ have been smeared out because $\Delta_{\pm}$ is angular dependent. 
\begin{figure}
    \centering
    %\subcaptionbox{
  %}[0.45\linewidth]
  %{\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Sigmar2Dnew27.png}}
  \includegraphics[width =8.4cm]{figures/Sigmar2Dnew27.png}
%\hfill
%\subcaptionbox{
%  }[0.45\linewidth]
%  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/SigmaRPdominantnew27.png}}
    \caption{The conductance of the s+$\text{p}_{\text{x}}$ junction for several values of $r$. The results are similar to the purely one-dimensional case, if the p-wave component is dominant there is a large zero bias conductance peak, if the s-wave component is dominant there is only a small peak around $E = 0$ on the scale of the Thouless energy \cite{blonder1982transition}, and disappears for short junctions. However, an important different with the purely one-dimensional case in \cite{tanaka2021phys} is that the height of the zero bias conductance peak now depends on the value of $r$, the addition of an s-wave component leads to a reduction of the peak height.}
    \label{fig:Sigma2D}
\end{figure}
\begin{figure}
    \centering
    \subcaptionbox{$r = 0$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/SigmaeVR$\text{p}_{\text{x}}$.png}}
\hfill
\subcaptionbox{$r = 0.2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/SigmaeV0$\text{p}_{\text{x}}$.png}}

    \caption{The conduction in the quasi-1D SNN junction with a mixed s + $\text{p}_{\text{x}}$-wave superconductor pair potential as a function of voltage and $\frac{r}{1+r}$. The distinction between the two cases is clearly visible. For $r<1$ there is a dip in the density of states at low energies, for $r>1$ there is a peak at low energies. The width of the peak or dip decreases as the contributions from the s-wave and p-wave component become more equal in strength. The conductance at zero energy does not show a discontinuity at $r = 1$.}
    \label{fig:SigmaeV$\text{p}_{\text{x}}$}
\end{figure}
\begin{comment}
\subsection{Numerical convergence}
The numerical errors of the procedure laid out above for solving the Usadel equation in quasi-one-dimensional junctions, was tested by performing the calculation for various gridsizes, the number of gridpoints $Nx$ was varied to be 101, 201, 401 and 801. In this paragraph, the solution at $Nx = 801$ is taken as the 'true' solution, and the other three solutions are compared with this solution. The quantities of interest are
\begin{align}
    \mathcal{E}_{\nu}(Nx,E) &= |\nu(Nx,E)-\nu(801,E)|.\\
    \mathcal{E}_{\chi}(Nx,E) &= |\chi(Nx,E)-\chi(801,E)|.\\
    Q_{\nu}(E) &= \frac{\mathcal{E}_{\nu}(101,E)-\mathcal{E}_{\nu}(201,E)}{\mathcal{E}_{\nu}(201,E)-\mathcal{E}_{\nu}(401,E)}\\
    Q_{\chi}(E) &= \frac{\mathcal{E}_{\nu}(101,E)-\mathcal{E}_{\nu}(201,E)}{\mathcal{E}_{\nu}(201,E)-\mathcal{E}_{\nu}(401,E)}
\end{align}
where $\nu(Nx,E)$ and $\chi(Nx,E)$ denote the solutions at the interface between the normal metal and the superconductor as calculated using $Nx$ grid points. The quantities $\mathcal{E}_{\nu}$ and $\mathcal{E}_{\chi}$ give the absolute error in the density of states, which is determined by the parameter $\theta$, and the parameter $\chi$, respectively, and indicate whether the numerical solution is already close to the 'true' solution. The values $Q_{\nu}$ and $Q_{\theta}$ are indicators of the order of convergence $p$, which can be calculated by $p_{\nu,\chi} = \log_{2}(Q_{\nu,\chi})$. The results are shown in figures \ref{fig:Errnu2D}, \ref{fig:Qnu2D}, \ref{fig:Errchi2D} and \ref{fig:Qchi2D}. It was found that for both the density of states and the parameter $\chi$ the differences between solutions as found with different grid sizes is at most of order $10^{-5}$, indicating that the number of grid points used in the calculation is large enough for an accurate solution. Moreover, the order of convergence was found to be 2, which is expected from the use of the discretisation scheme including the ghost cell boundary method.
\begin{figure}
    \centering
    \subcaptionbox{$r = 0.2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Errnu0p2.png}}
\hfill
\subcaptionbox{$r = 0.9$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Errnu0p9.png}}
\hfill
\subcaptionbox{$r = 2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Errnu2.png}}
\hfill
\subcaptionbox{$r = 10$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Errnu10.png}}
    \caption{The difference between the density of states at the interface as calculated using $Nx = 801$ and $Nx\in\{101, 201, 401\}$. The differences are at most of order $10^{-5}$ over the whole energy range, indicating that the numerical grid if fine enough for reliable calculations. The numerical errors are slightly larger if $r>1$ then if $r<1$.}
    \label{fig:Errnu2D}
\end{figure}

\begin{figure}
    \centering
    \subcaptionbox{$r = 0.2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Qnu0p2.png}}
\hfill
\subcaptionbox{$r = 0.9$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Qnu0p9.png}}
\hfill
\subcaptionbox{$r = 2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Qnu2.png}}
\hfill
\subcaptionbox{$r = 10$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Qnu10.png}}
    \caption{The Q-value for the density of states at the interface for four different values of $r$. The Q-value is mostly close to 4, indicating a second order convergence. Near zero energy the order of convergence becomes less well defined. The reason for this is that the actual solution to the differential equation solved is almost linear. Therefore, the main source of error is not the discretisation of the interval, but rather errors that are due to the MATLAB accuracy. This is consistent with the very small error at low energies as found in figure \ref{fig:Errnu2D}.}
    \label{fig:Qnu2D}
\end{figure}

\begin{figure}
    \centering
    \subcaptionbox{$r = 0.2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Errchi0p2.png}}
\hfill
\subcaptionbox{$r = 0.9$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Errchi0p9.png}}
\hfill
\subcaptionbox{$r = 2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Errchi2.png}}
\hfill
\subcaptionbox{$r = 10$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Errchi10.png}}
    \caption{The difference between the parameter $\chi$ as calculated using $Nx = 801$ and $Nx\in\{101, 201, 401\}$. The differences are at most of order $10^{-6}$, indicating that the numerical grid if fine enough for reliable calculations. There is no clear difference between the magnitude of the numerical error for $r<1$ and $r>1$ respectively.}
    \label{fig:Errchi2D}
\end{figure}

\begin{figure}
    \centering
    \subcaptionbox{$r = 0.2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Qnu0p2.png}}
\hfill
\subcaptionbox{$r = 0.9$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Qnu0p9.png}}
\hfill
\subcaptionbox{$r = 2$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Qnu2.png}}
\hfill
\subcaptionbox{$r = 10$
  }[0.45\linewidth]
  {\hspace*{-2em}\includegraphics[width =8.4cm]{figures/Qnu10.png}}
    \caption{The Q-value for the parameter $Q$ at the interface for four different values of $r$. The Q-value is mostly close to 4, indicating a second order convergence. Thus, the order of convergence for $\chi$ is the same as the order of convergence for $\theta$.}
    \label{fig:Qchi2D}
\end{figure}
\end{comment}
